Annotators with Attitudes: How Annotator Beliefs And Identities Bias Toxic Language Detection

The perceived toxicity of language can vary based on someone's identity and beliefs, but this variation is often ignored when collecting toxic language datasets, resulting in dataset and model biases. We seek to understand the who, why, and what behind biases in toxicity annotations. In two online studies with demographically and politically diverse participants, we investigate the effect of annotator identities (who) and beliefs (why), drawing from social psychology research about hate speech, free speech, racist beliefs, political leaning, and more. We disentangle what is annotated as toxic by considering posts with three characteristics: anti-Black language, African American English (AAE) dialect, and vulgarity. Our results show strong associations between annotator identity and beliefs and their ratings of toxicity. Notably, more conservative annotators and those who scored highly on our scale for racist beliefs were less likely to rate anti-Black language as toxic, but more likely to rate AAE as toxic. We additionally present a case study illustrating how a popular toxicity detection system's ratings inherently reflect only specific beliefs and perspectives. Our findings call for contextualizing toxicity labels in social variables, which raises immense implications for toxic language annotation and detection.

==> 8-discussion-old.tex <==
\section{Discussion \& Conclusion}
\label{sec:discussion}



Overall, our analyses showed that perceptions of toxicity are indeed affected by readers' demographic identities and beliefs (\S\ref{sec:whowhatwhy}).
We showed---via both a \smallscale study and a \largescale study (\S\ref{sec:study-designs})---several associations when isolating specific text characteristics: \racist (\S\ref{sec:racist-results}), \AAE (\S\ref{sec:AAE-results}), and \vulgarity (\S\ref{sec:vulgar-results}); see full, detailed results in Appendix \S\ref{sec:smallScale-more} and \S\ref{app:largeScale-results}. %\swabha{added this so they can see the full results summarized in tables 10 and 11.}\maarten{sgtm}
Finally, we showed that a popular toxicity detection system produces toxicity scores that are more aligned with raters with certain attitudes and identities than others (\S\ref{sec:perspective-main}).
We discuss implications of our findings below.

\paragraph{Collect annotator identities and attitudes.}
Given that many NLP tasks are increasingly socially or politically laden (misinformation, hate speech, stereotypes, biased language, etc.), it is important to consider who is annotating data and what their beliefs are about the task. 
While several works have recruited or subselected annotators to hold particular ideologies \cite[e.g.,][]{waseem2016you,sap2020socialbiasframes,vidgen-etal-2021-learning}, annotator attitudes are only vaguely described.
We advocate for collecting attitude scores based on relevant social science research, perhaps in lightweight format as done in our \largescale study, and reporting those scores along with the dataset \cite[e.g., in datasheets;][]{gebru2018datasheets}.

% \maarten{We should mention that some work has definitely already recruited or subselected annotators to hold particular ideologies \cite[e.g.,][]{waseem2016you,sap2020socialbiasframes,vidgen-etal-2021-learning}},  there isn't much concrete evidence of what their attitudes are towards specific 
% }

% \paragraph{Who decides what is toxic?}

\paragraph{Contextualize toxicity predictions in social variables.}
As shown in our results and previous studies \cite[e.g.,][]{waseem2016you,Ross2017measuring,waseem2021disembodied}, determining what is toxic is subjective.
However, given this subjectivity, the open question remains: whose perspective should be considered when using toxicity detection models? 
To try answering this question, we urge researchers and practitioners to consider all stakeholders and end users on which toxicity detection systems might be deployed \cite{sanders2002user,friedman2008value,hovy-yang-2021-importance}.
Additionally, we urge people to embrace that each design decision has socio-political implications \cite{green2020political,cambo2021model}, and encourage them to develop technologies to shift power to the targets of oppression \cite{blodgett-etal-2020-language,Kalluri2020-jk,Birhane2021-ui}.
Finally, given the increasingly essential role of online platforms in people's daily lives \cite{Rahman2017-la}, we echo calls for policy regulating these toxicity detection algorithms \cite{Jiang2020-qv,McGuffie2020radicalization}.%Gillespie2020-wd,

% \paragraph{Beyond binary decisions}
% Our findings corroborate previous findings that phrasing an offensiveness question differently can yield different annotation sensitivities \cite{sap-etal-2019-risk}.
% \swabha{add more}

\paragraph{Think beyond classification: modeling distributions and explanations.}
Our findings on the subjectivity of the toxicity detection tasks suggests that standard approaches of obtaining binary (or even $n$-ary) labels of toxicity and averaging them into a majority vote are inadequate.
Instead, researchers could consider modeling the distribution or variation in toxicity labels with respect to individual annotators \cite{geva-etal-2019-modeling,fornaciari-etal-2021-beyond,Davani2021-md} or to specific identities or beliefs.
% We advocate for more holistic frameworks for representing toxicity. 

But, perhaps more importantly, we encourage rethinking the toxicity detection paradigm altogether.
If the goal is to assist human content moderators, making our systems explain biased implications of statements could be more helpful than opaque toxicity scores \cite{Gillespie2020-wd}.
Therefore, we advocate for moving away from classification frameworks, and towards more nuanced, holistic, and explainable frameworks for inferring the desired concepts of toxicity and social biases \cite[e.g., the hierarchical Social Bias Frames formalism;][]{sap2020socialbiasframes}.

\section*{Further Ethical Considerations}
\maarten{Re-summarize that we treated the crowdworkers }
\maarten{Add a limitations section maybe?}

\paragraph{Limitations}
\maarten{scales used may need extra validation. Additionally, other empathy scales could be used \cite{gerdes2011measuring}.}


% seeking majority votes to determine (often, binary) toxicity labels for text is inadequate.
% Moreover, the typical classification framework used for this task encourages impression-based thinking. \maarten{- this last sentence is not great haha so feel free to remove} \nascomment{agree, cut it; other stuff is clearer and more powerful}
% If the goal is to assist human content moderators, making our systems explain biased implications of statements could be more helpful than opaque toxicity scores.

% With content moderation in mind, the most useful tools are the ones that assist human moderators, for example by generating explanations \cite{Gillespie2020-wd}.


% \swabha{Takeaway 1: Use more annotators, and diverse! Selection of annotators based on some criteria has been explored in \cite{thakur2021mixed}. 
% Diverse perspectives help models \cite{kumar2021designing}. From Gardner contrast sets: biases due to the writing styles of small groups of annotators \cite{geva-etal-2019-modeling}, the distributional biases in the data that was chosen for annotation, as well as numerous other biases that are more subtle and harder to discern \cite{shah2020predictive}.}
% \maarten{I'm not sure that ``diverse'' pool is everyone's goal? Not sure how to incorporate that...}


% \maarten{I took your points and started incorporating them into some paragraphs, but still needs work, and needs at least one more paragraph}
% \swabha{Takeaway 2: Collect attitudes and demographics to ensure diverse pool.} \maarten{Moved that to point number 1 above}


% \swabha{Takeaway 3: Consider non-prescriptive models, i.e look beyond classification}

% \swabha{Takeaway 4: We conclude that labels cannot be simple, and are very dependent on the annotators.}

% \swabha{Overall, we must embrace the politics behind these design decisions \cite{green2020political,cambo2021model}.}



% \swabha{removing limitations for now, to be revisited }
% \subsection{Limitations}
% \label{ssec:discussion-limitations}

% \swabha{\smallscale didn't account for vulgar OI, didn't consider age, country of origin. Only kinds of racism are anti-Black, and there is an assumption that \AAE cannot be \racist.}
% Future work could consider additional attributes such as annotator age, sexual orientation etc, for both small- and large-scale studies.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \maarten{
% AAE isn't inherently considered offensive if it has no vulgar or profane words. However, several common markers of AAE (``\textit{n*gga}'', the ``\textit{-ass}'' suffix) could be considered obscene or profane in themselves \cite{spears1998african}.
% We probably should have added a 4th category of AAE with those reclaimed slurs and -ass suffixes \cite{zhou2021challenges}, to investigate how those compare?
% }

% \maarten{
% \AAE connotes blackness?
% We found that annotator racism (ERB) correlated with annotating AAE tweets as racist!
% Also, AAE was rated as more racist than Vulgar on average, an effect which seems to be present specifically for whites and liberals.
% This suggests that somehow annotators can understand that AAE is associated with the Black racial identity, as language is known to convey race \cite{Rosa2019soundingLikeRace}.
% This could be related to this weird idea that mentioning someone's race is racist \cite[colorblind racism;][]{bonilla2006colorblindRacism}?
% Linking this to \citet{sap-etal-2019-risk}, who show that giving the race or dialect of the tweet can decrease the ratings of offensiveness, so maybe this effect would not have been present if we had indicated that the tweets were AAE?
% }
% \paragraph{Political attitudes have a strong effect}
% \maarten{Our strongest finding is that someone's attitudes about race, free speech, and hate speech, and overall political leaning \textbf{strongly} correlate with how offensive they perceive \racist tweets to be.
% It's widely established that conservative voters in the US tend to hold more racist attitudes \cite{Goldstein2017-mx,Lucks2020-ri,Schaffner2020-jv}, especially in the Trump era of politics.
% Also, it's been kind of established that empathy, altruism, and harm of hate speech correlate \cite{cowan2003empathy}.
% Taking it together, it just seems like political leaning is an incredibly necessary variable to take into account when considering content moderation and offensiveness annotations.
% People who make hate speech detection tools should choose annotators that align with the goals of the research \cite{waseem2016you,vidgen-etal-2021-learning}: if it's to find and flag racist content, they should be really careful because racist annotators will miss a lot of posts.
% }







==> annotatorAttitudesIdentities-Laura.tex <==

As online communication becomes the norm, social media platforms encounter the challenge of keeping their online content free of toxic language (e.g., hate speech, abusive speech, or other offensive speech). Many researchers have shown that automated speech detection tools are limited due to the complexity and subjectivity of what is considered toxic language and what is not (cite). Most datasets for hate speech detection still use simplified notions of toxicity, such as binary or ternary labels indicating whether or not a piece of text contains offensive text. These labels are aggregated over (using simple averages) judgments of multiple human annotators, regardless of who the annotators are, and what their beliefs are. Furthermore, automated tools carry biases from annotators (Zampieri et al., 2019). Therefore, a comprehensive understanding of the demographics and psychological attitudes of annotators is necessary to unpack biases in toxic language detection. This results in disparate impacts of automatic speech moderation, for instance among speakers of minority dialects, such as African American Vernacular English (AAVE) speakers. Indeed, Sap et al. (2019) showed that simply priming human annotators about the dynamics of in-group AAVE speech substantially improves the quality of annotations. (sentence here….)(Zampieri et al., 2019).
In order to comprehend biases in automatic speech detection, it’s necessary to understand the biases that annotators introduce to the process. (Past lit on annotator biases for next sentences? An annotation task may introduce many sources of bias, such as by priming annotators (or something like this?)). 

Vulgar Language 

People have strong reactions to vulgarity in language and make snap decisions based on the emotional charge of the vulgarity used. Indeed, people are quick to rate speakers of the vulgar language as less likable and less trustworthy than those who don’t use vulgar language (DeFrank & Kahlbaugh1, 2019).  Due to the emotional charge of vulgar language, annotators may conflate offensive language with anything that contains vulgar language, or profanity (Zampieri et al., 2019).), 
.

Psychological factors behind annotators judgments of offensiveness

The Role of Annotators

Annotators are not a monolith. Demographic factors (e.g., race, gender, political orientation) and annotators’ attitudes and belief systems shape their labeling of what is toxic language and what is not. If automated speech detection tools are trained on a sample of annotators of a particular group, the tools will also be biased; resulting in either underestimation or overestimation of what is considered toxic language or not (or incongruities with the goals of speech detection). For example, someone who is highly traditional may label a mild obscenity as very toxic, resulting in an overestimation error. In contrast, those who are not as traditional may label a tweet with stronger obscenity as not at all toxic, resulting in an underestimation error. In this work, we attempt to identify potential demographic variables and psychological attitudes (or belief systems) that may introduce biases in speech detection of toxic language. 



Traditionalism

Adherence to societal traditional values is often opposed to the acceptability of vulgar language (Sapolsky et al., 2011). We predicted that highly traditional annotators would rate tweets that contained vulgar language as offensive because it directly goes against their moral values. We used an adapted version of the Traditionalism scale (Bouchard et al., 2003) to measure annotators' adherence to traditional values.  

(Bouchard Jr, T. J., Segal, N. L., Tellegen, A., McGue, M., Keyes, M., & Krueger, R. (2003). Evidence for the construct validity and heritability of the Wilson–Patterson conservatism scale: A reared-apart twins study of social attitudes. Personality and Individual Differences, 34(6), 959-969.)

Language purism

Language purism - the usually exaggerated commitment to upholding the ‘correct’ use of language - may also affect how people rate vulgar language. Vulgar language is often not understood as a canonical part of the English language (cite?) (Sapolsky et al., 2011; DeFrank & Kahlbaugh1, 2019)  Therefore, we hypothesized that language purism could predict higher ratings of vulgar language as offensive.In order to measure language purism, we created items and validated with two research assistants. 

Racism

Racial prejudice often correlates with less likelihood to accept the term ‘hate speech’ (Roussos, G., & Dovidio, J. F. (2018).). Social threat theory, for example, frames this reluctance as a form of threat of being individually seen as racist, or their group is seen as racist (Duckitt, J., & Fisher, K. (2003).). Therefore, we theorized that annotators’ endorsement of anti-minority attitudes would predict reluctance to label hate speech as offensive. We used items from the validated 'Modern Racism Scale' to measure annotators' endorsement of racist beliefs - or anti-minority beliefs.  




Empathy

Research in Social Psychology has linked higher levels of empathy to recognize and label hate speech (Cowan, G., & Khatchadourian, D. (2003).). The relationship between empathy and labeling anti-minority speech as hate speech may happen because sensitivity and responsiveness to the needs and feelings of others include heightened sensitivity to interpersonal infringement (Inman, M. L., & Baron, R. S. (1996). Therefore, we theorize that highly empathic annotators would be more likely to label hate speech as offensive.  


The Offensiveness of Hate Speech

Americans are known to express great endorsement of free speech and reluctance to label hate speech. Various psychological theories provide insight into what causes this reluctance. Here we attempt to predict annotators’ likelihood of labeling anti-minority language (hate speech) as offensive. 

The Harm of Hate Speech and Endorsement of Free Speech

Recognizing hate speech as harmful is directly opposed to upholding free speech beliefs when free speech is threatened by censorship (Downs, D. M., & Cowan, G. (2012).). Therefore, we predicted that annotators who place a higher value on unrestricted speech (free speech) would be reluctant to label any speech as offensive, due to fear of censorship (Cole, D. (1996).

Similarly, we predicted that annotators who don't believe that offensive speech can harm minorities, would be less likely to label tweets in the racially offensive category as offensive. 
-------
References

Sapolsky*, B. S., Shafer, D. M., & Kaye, B. K. (2010). Rating Offensive Words in Three Television Program Contexts. Mass Communication and Society, 14(1), 45–70. 
https://www.tandfonline.com/doi/abs/10.1080/15205430903359693

Zampieri, M., Malmasi, S., Nakov, P., Rosenthal, S., Farra, N. & Kumar, R. (2019). Predicting the Type and Target of Offensive Posts in Social Media. 1415-1420. 
https://arxiv.org/pdf/1902.09666.pdf

DeFrank, M. & Kahlbaugh, P. (2018). Language Choice Matters: When Profanity Affects How People Are Judged. Journal of Language and Social Psychology. 38. 0261927X1875814. 
https://journals.sagepub.com/doi/pdf/10.1177/0261927X18758143

Roussos, G., & Dovidio, J. F. (2018). Hate speech is in the eye of the beholder: The influence of racial attitudes and freedom of speech beliefs on perceptions of racially motivated threats of violence. Social Psychological and Personality Science, 9(2), 176-185.

Duckitt, J., & Fisher, K. (2003). The impact of social threat on worldview and ideological attitudes. Political Psychology, 24(1), 199-222.

Cowan, G., & Khatchadourian, D. (2003). Empathy, ways of knowing, and interdependence as mediators of gender differences in attitudes toward hate speech and freedom of speech. Psychology of Women Quarterly, 27(4), 300-308.

Inman, M. L., & Baron, R. S. (1996). Influence of prototypes on perceptions of prejudice. Journal of Personality and Social Psychology, 70, 727–739.

Downs, D. M., & Cowan, G. (2012). Predicting the importance of freedom of speech and the perceived harm of hate speech. Journal of applied social psychology, 42(6), 1353-1375.

Cole, D. (1996) Racist speech should be protected by the constitution. In P. A. Winters (Ed.), Hate crimes(pp. 89–96). San Diego, CA: Greenhaven.

Gaither, S. E., Cohen-Goldberg, A. M., Gidney, C. L., & Maddox, K. B. (2015). Sounding Black or White: Priming identity and biracial speech. Frontiers in Psychology, 6, 457.

McConahay, J. B. (1986). Modern racism, ambivalence,
and the modern racism scale. In J. F. Dovidio & S. L.

Gaertner (Eds.), Prejudice, discrimination, and racism
(pp. 91–125). London: Academic Press.

Waseem, Z., & Hovy, D. (2016, June). Hateful symbols or hateful people? predictive features for hate speech detection on twitter. In Proceedings of the NAACL student research workshop (pp. 88-93).

Al Kuwatly, H., Wich, M., & Groh, G. (2020, November). Identifying and measuring annotator bias based on annotators’ demographic characteristics. In Proceedings of the Fourth Workshop on Online Abuse and Harms (pp. 184-190).

Poteat, V. P., & Spanierman, L. B. (2012). Modern racism attitudes among White students: The role of dominance and authoritarianism and the mediating effects of racial color-blindness. The Journal of Social Psychology, 152(6), 758-774.

Pulos, S., Elison, J., & Lennon, R. (2004). The hierarchical structure of the Interpersonal Reactivity Index. Social behavior and personality, 32(4), 355-360.

Bouchard Jr, T. J., Segal, N. L., Tellegen, A., McGue, M., Keyes, M., & Krueger, R. (2003). Evidence for the construct validity and heritability of the Wilson–Patterson conservatism scale: A reared-apart twins study of social attitudes. Personality and Individual Differences, 34(6), 959-969. (??????)

Downs, D. M., & Cowan, G. (2012). Predicting the importance of freedom of speech and the perceived harm of hate speech. Journal of applied social psychology, 42(6), 1353-1375.

Nelson, J. C., Adams, G., & Salter, P. S. (2013). The Marley hypothesis: Denial of racism reflects ignorance of history. Psychological science, 24(2), 213-218.

Gavrilets, S., & Fortunato, L. (2014). A solution to the collective action problem in between-group conflict with within-group inequality. Nature communications, 5(1), 1-11.

Riar, M., Morschheuser, B., Hamari, J., & Zarnekow, R. (2020, January). How game features give rise to altruism and collective action? Implications for cultivating cooperation by gamification. In Proceedings of the 53rd Hawaii International Conference on System Sciences.

Cowan, G., Resendez, M., Marshall, E., & Quist, R. (2002). Hate speech and constitutional protection: Priming values of equality and freedom. Journal of Social Issues, 58(2), 247-263.



--------
Meeting 10/04 notes

Altruism -> associated wiuth hate speech 

==> tables/tab-overall.tex <==
\begin{table*}[t!]
    \footnotesize
    \centering
    \begin{tabular}{lp{4cm}p{3.5cm}p{3.5cm}}
        \toprule
        & \bf \Smallscale & \bf \Largescale & \bf \Largescale-Overlap \\
        \midrule
        \multicolumn{4}{c}{\bf \Racist}\\
        \midrule
        \textit{Rated as Offensive} 
        & \empathy, \altruism, \harmOfHateSpeech, \freeSpeech, \racistBeliefs, \lingPurism, \traditionalism, Politics, Gender, Race
        & \harmOfHateSpeech, \freeSpeech, \racistBeliefs
        & \harmOfHateSpeech, \racistBeliefs \\
        \midrule[0.03em]
        \textit{Rated as Racist}
        & \empathy, \altruism, \harmOfHateSpeech, \freeSpeech, \racistBeliefs, \lingPurism,
        \traditionalism, Politics, Gender
        & \freeSpeech, \racistBeliefs
        & \harmOfHateSpeech, \freeSpeech, \racistBeliefs \\
        \midrule
        \multicolumn{4}{c}{\bf \AAE}\\
        \midrule[0.03em]
        \textit{Rated as Offensive} 
        & ---
        & ---
        & \racistBeliefs, \traditionalism, Politics\\
        \midrule[0.03em]
        \textit{Rated as Racist}
        & \racistBeliefs, Politics
        & \freeSpeech, Politics, Race
        & \freeSpeech, Politics, \traditionalism \\
        \midrule
        \multicolumn{4}{c}{\bf \Vulgar}\\
        \midrule[0.03em]
        \textit{Rated as Offensive} 
        & \lingPurism, \traditionalism, Politics
        & \empathy, \altruism, \harmOfHateSpeech, \freeSpeech, \traditionalism
        & \textbf{\OnI:} Politics; \textbf{\OI:} \empathy, \harmOfHateSpeech, \traditionalism \\
         \midrule[0.03em]
        \textit{Rated as Racist}
        & ---
        & ---
        & \textbf{\OnI:} Politics; \textbf{\OI:} Politics \\
         \midrule
        \bottomrule
    \end{tabular}
    \caption{Summary of Results: only significant ($p > $ \swabha{todo}) associations reported.}
    \label{tab:overall}
\end{table*}
